Bayes-TrEx: a Bayesian Sampling Approach to Model Transparency by Example

Post-hoc explanation methods are gaining popularity for interpreting, understanding, and debugging neural networks. Most analyses using such methods explain decisions in response to inputs drawn from the test set. However, the test set may have few examples that trigger some model behaviors, such as high-confidence failures or ambiguous classifications. To address these challenges, we introduce a flexible model inspection framework: Bayes-TrEx. Given a data distribution, Bayes-TrEx finds in-distribution examples with a specified prediction confidence. We demonstrate several use cases of Bayes-TrEx, including revealing highly confident (mis)classifications, visualizing class boundaries via ambiguous examples, understanding novel-class extrapolation behavior, and exposing neural network overconfidence. We use Bayes-TrEx to study classifiers trained on CLEVR, MNIST, and Fashion-MNIST, and we show that this framework enables more flexible holistic model analysis than just inspecting the test set. Code is available at https://github.com/serenabooth/Bayes-TrEx.

==> appendices/ethics.tex <==
\section{Ethics Statement}
\label{da-ethics}


\textsc{Bayes-TrEx} has potential to allow humans to build more accurate mental models of how neural networks make decisions. Further, \textsc{Bayes-TrEx} can be useful for debugging, interpreting, and understanding networks---all of which can help us build \emph{better}, less biased, increasingly human-aligned models. 

However, \textsc{Bayes-TrEx} is subject to the same caveats as typical software testing approaches: the absence of exposed bad samples does not mean the system is free from defects. One concern is how system designers and users will interact with \textsc{Bayes-TrEx} in practice. If \textsc{Bayes-TrEx} does not reveal degenerate examples, these stakeholders might develop inordinate trust~\cite{lee2004trust} in their models.

Additionally, one \textsc{Bayes-TrEx} use case is to generate examples to be used as inputs to downstream local explanation methods. As a community, we know that many of these local explanations can be challenging to understand~\cite{olah2017feature,nguyen2019understanding}, misleading~\cite{adebayo2018sanity,kindermans2019reliability,rudin2019stop}, or susceptible to adversarial attacks~\cite{slack2019can}. In human-human interaction, even nonsensical explanations can increase compliance~\cite{langer1978mindlessness}. As we build post-hoc explanation techniques, we must evaluate whether the produced explanations help humans moderate trust and act appropriately---for example, by overriding the model's decisions. 

